Some results on order bounded almost weak Dunford-Pettis operators

We give some new characterizations of almost weak Dunford-Pettis operators and we investigate their relationship with weak Dunford-Pettis operators.

==> jinfo.tex <==
\jvolume{22}
\jyear{2016}
\jnumber{3}

